Scalable Similarity Search for Molecular Descriptors

Similarity search over chemical compound databases is a fundamental task in the discovery and design of novel drug-like molecules. Such databases often encode molecules as non-negative integer vectors, called molecular descriptors, which represent rich information on various molecular properties. While there exist efficient indexing structures for searching databases of binary vectors, solutions for more general integer vectors are in their infancy. In this paper we present a time- and space- efficient index for the problem that we call the succinct intervals-splitting tree algorithm for molecular descriptors (SITAd). Our approach extends efficient methods for binary-vector databases, and uses ideas from succinct data structures. Our experiments, on a large database of over 40 million compounds, show SITAd significantly outperforms alternative approaches in practice.

==> abst.tex <==
\begin{abstract}
Similarity search over chemical compound databases is a fundamental task in the discovery and design of novel drug-like molecules. Such databases often encode molecules as non-negative integer vectors, called {\em molecular descriptors}, which represent rich information on various molecular properties. 
%The succinct interval-splitting tree (SITA) (Tabei et al., KDD'13) 
While there exist efficient indexing structures for searching databases of {\em binary} vectors, solutions for more general integer vectors are in their infancy. 
In this paper we present a time- and space-efficient index for the problem that we call the {\em succinct intervals-splitting tree algorithm for molecular descriptors (SITAd)}. Our approach extends efficient methods for binary-vector databases, and uses ideas from succinct data structures.
Our experiments, on a large database of over $40$ million compounds, show SITAd significantly outperforms alternative approaches in practice.
%We experimentally test SITAd on the ability to retrieve similar compounds for a query from a large database with over $40$ million compounds and 
%show that SITAd performs better than other possible approaches.
\end{abstract}


==> review.tex <==
\section{Literature review}
Several efficient methods have been proposed for similarity search of {\em molecular fingerprints} defined as binary vector, 
where Tanimoto similarity (a.k.a Jaccard similarity) has been used. 
To our knowledge, most of the state-of-the-art methods defines a bound of Tanimoto similarity and 
prunes the search space by using the bound to reduce the number of similarity calculations. 

Early work by Swamidas and Baldi~\cite{} derives a bound of Tanimoto similarity from the number of on-bits in fingerprints. 
Baldi et al.~\cite{} derived a tight bounder based on an exclusive-OR approach. 
Recently, essential identical idea was proposed in three independent papers. 
Their idea is to divide fingerprints into several blocks and 
define a bound in each block by the Swamidas and Baldi's method~\cite{}.
With this bound, Christensen et al.~\cite{} proposed tree based data structures 
for similarity search. 

Recently, molecular descriptor, defined as integer vector, has commonly been used for similarity search of chemical compounds. 
Representative molecular descriptors are LINGO~\cite{} and KCF-S~\cite{}. 
Kristensen et al.~\cite{} proposed the first similarity search of chemical descriptors using inverted index, 
which is an associative array whose key is an element of descriptor and value is a descriptor identifier. 
The efficiency of their similarity search has only been shown on a small database of LINGO descriptors, 
However, inverted index uses a large amount of memory to store a large database of chemical descriptors, e.g., PubChem.  
One can compress an inverted index using compression methods for inverted index, but decompressing the compressed inverted index 
takes a long time, resulting in a large time of similarity search. 



% アウトライン
% descriptors (integer vector)の類似度検索手法が重要
% Kristensen et al.がinverted index based methodを提案した。
% しかし、メモリー使用量が大きい
% inverted indexを圧縮すると検索速度が遅くなる
% メモリーと検索速度を両立する手法がほしい





